On-the-fly Table Generation

Many information needs revolve around entities, which would be better answered by summarizing results in a tabular format, rather than presenting them as a ranked list. Unlike previous work, which is limited to retrieving existing tables, we aim to answer queries by automatically compiling a table in response to a query. We introduce and address the task of on-the-fly table generation: given a query, generate a relational table that contains relevant entities (as rows) along with their key properties (as columns). This problem is decomposed into three specific subtasks: (i) core column entity ranking, (ii) schema determination, and (iii) value lookup. We employ a feature-based approach for entity ranking and schema determination, combining deep semantic features with task-specific signals. We further show that these two subtasks are not independent of each other and can assist each other in an iterative manner. For value lookup, we combine information from existing tables and a knowledge base. Using two sets of entity-oriented queries, we evaluate our approach both on the component level and on the end-to-end table generation task.

==> 00paper-11.tex <==
\section{Evaluation}
In this section, we discuss our experimental setup, present the results of different iterations and  
\section{Results and analysis}

\sz{Evaluation: use the test collections or the original WP table for evaluation. Methods: entity and attributes, two directions. If use WP tables as KB, evaluation on schema should be different cuz they are along with the entites.}



\subsection{Entity retrieval Evaluation}

\begin{table*}[t]
\center
\caption{Entity retrieval results for query sets.\sz{ top-$k$ means  top-$k$ results from last round schema determination}}
	\begin{tabular}{lccccc}
	\toprule
%	& \multicolumn{5}{c}{\textbf{Query set}} \\
%	 & \multicolumn{2}{c}{\textbf{QS1}} & \multicolumn{2}{c}{\textbf{QS2}} \\
%	 \midrule
	 
    	& \multicolumn{2}{c}{\textbf{QS1}} && \multicolumn{2}{c}{\textbf{QS2}} \\
    \cline{2-3} \cline{5-6} 
    \textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} & &
    \textbf{NDCG@5} & \textbf{NDCG@10}  \\

	\midrule
%	\textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10}& \textbf{NDCG@5} & \textbf{NDCG@10} \\
%	\midrule
	(1) LM & 0.2419 & 0.2591 && 0.0708 & 0.0823 \\
	(2) TKS\_QE & 0.2015 & 0.2028 && 0.0501 & 0.0540 \\
	(3) TKS\_QP & 0.1780 & 0.1808 && \textbf{0.1089} & \textbf{0.1083} \\
	(1) + (2) & 0.2578 & 0.2620 && 0.0619 & 0.0686  \\
	(1) + (3) & 0.2562 & 0.2713 && 0.0906 & 0.1004 \\
	(1) + (2) + (3) & \textbf{0.2821} & \textbf{0.2834} && 0.0852 & 0.0920 \\
%	(4) TKS\_SP & 0.1645 & 0.1703 \\
	\midrule
	(4) TKS\_SP* & 0.1645 & 0.1703 && 0.1320 & 0.1318 \\
	(5) TKS\_SE* & 0.1672 & 0.1660 && 0.1096 & 0.1086 \\
	(6) TKS\_QSEP* & 0.2039 & 0.2002 && 0.0357 & 0.0386 \\
	(7) cc* & 0.1816 & 0.1844 && 0.1551 & 0.1512 \\	
	(1) + (2) + (3) + (4)* & 0.3071 & 0.3055 && 0.1234 & 0.1208 \\
	(1) + (2) + (3) + (5)* & 0.2935 & 0.2887 && 0.1038 & 0.1024 \\
	(1) + (2) + (3) + (6)* & 0.2887 & 0.2812 && 0.0913 & 0.0924 \\
	(1) + (2) + (3) + (7)* & 0.3404 & 0.3319 && 0.1467 & 0.1475\\
	All & \textbf{0.3518} & \textbf{0.3355} && \textbf{0.1587} & \textbf{0.1555} \\ % DB: all (-se); ER: cc + sp
	\midrule
	round2 top5 & 0.2892 & 0.2842 && 0.1198 & 0.1166\\
	round2 top10 & 0.3012 & 0.2892 && 0.1232 & 0.1201 \\
	round2 top20 & 0.2923 & 0.2905 && 0.1222 & 0.1174\\
	\midrule
	round3 top5 & 0.3259 & 0.3105 && 0.1260 & 0.1258\\ %db:-f
	round3 top10 & 0.3369 & 0.3221 && 0.1307 & 0.1264 \\
	round3 top20 & 0.3314 & 0.3219 && 0.1260 & 0.1242\\
	\bottomrule	
	\end{tabular}	
\label{tbl:er_qs}
\end{table*}

\begin{table*}[t]
\center
\caption{Entity retrieval results for query sets.\sz{ top-$k$ means  top-$k$ results from last round schema determination}}
	\begin{tabular}{lccccc}
	\toprule
%	& \multicolumn{5}{c}{\textbf{Query set}} \\
%	 & \multicolumn{2}{c}{\textbf{QS1}} & \multicolumn{2}{c}{\textbf{QS2}} \\
%	 \midrule
	 
    	& \multicolumn{2}{c}{\textbf{QS1}} && \multicolumn{2}{c}{\textbf{QS2}} \\
    \cline{2-3} \cline{5-6} 
    \textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} & &
    \textbf{NDCG@5} & \textbf{NDCG@10}  \\

	\midrule
	(1) + (2) + (3) & 0.2523 & 0.2653 && 0.1003 & 0.1048 \\
%	(4) TKS\_SP & 0.1645 & 0.1703 \\
	\midrule
%	All & 0.3026 & 0.3056 && 0.1728 & 0.1630 \\ % DB: all (-se); ER: cc + sp
%	\midrule
	round2 top5 & 0.2815 & 0.2803 && 0.1275 & 0.1241\\
	round2 top10 & 0.2782 & 0.2772 && 0.1308 & 0.1252 \\
	round2 top20 & 0.2907 & 0.2931 && 0.1296 & 0.1259\\
%	\midrule
%	round3 top5 & 0.3089 & 0.3083 && 0.1373 & 0.1314\\ %db:-f
%	round3 top10 & 0.3224 & 0.3203 && 0.1367 & 0.1323 \\
%	round3 top20 & 0.3101 & 0.3103 && 0.1331 & 0.1309\\
	\bottomrule	
	\end{tabular}	
\label{tbl:er_qs1}
\end{table*}

%\begin{table}[t]
%\center
%\caption{Entity retrieval results for query set 1 (DB).}
%	\begin{tabular}{lccc}
%	\toprule
%	\textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
%	\midrule
%%	BM25 & 0.2166 & 0.5429 & 0.2706 \\
%%	BM25-CA & 0.3136 & 0.6990 & 0.3709 \\
%%	BM25F-CA & \textbf{0.3323} & \textbf{0.7482} & \textbf{0.3914} \\
%%	FSDM-ELR & 0.3227 & 0.7240 & 0.3879 \\
%%	FSDM & 0.3141 & 0.7128 & 0.3783 \\
%%	LM Faegheh & 0.2899 0.2651 & 0.6915 & 0.3531 \\
%%	LM-ELR & 0.2977 & 0.7037 & 0.3636\\
%%	MLM-ALL & 0.2815 & 0.6985 & 0.3381 \\
%%	MLM-CA & 0.3050 & 0.7143 & 0.3662\\
%%	PRMS & 0.2728 & 0.7071 & 0.3380 \\
%%	SDM & 0.2958 & 0.6832 & 0.3513 \\
%%	SDM-ELR & 0.3059 & 0.3059 & 0.3636 \\
%%	\midrule
%%	LM using API & 0.2450 & 0.6445 & 0.3094 \\
%%	LM using API (stopped) & 0.2765 0.2535 & 0.6980 & 0.3508 \\
%	
%%	DSSM (only abstract) & 0.1700 & 0.1704 \\
%%	CDSSM (only abstract) & 0.1644 & 0.1762 \\
%%	DSSM (abstract + category) & 0.1726 & 0.1825 \\
%%	DRRM (only abstract) & 0.1816 & 0.1861 \\
%%	DSSM (abstract + category) & 0.1889 & 0.1991 \\
%%	DRRM (catchall) & 0.2561 & 0.2605 \\
%%	DRRM (5-cross...average 5 models) & 0.2678 & 0.2839 \\
%%	CDSSM & 0.0752 & 0.0776 \\
%%	DRMM (5-cross...each predict 20\%) & 0.0648 & 0.0743 \\
%%	DRMM(exclude gt from train) & 0.1645 & 0.1799 \\
%	
%	DRMM\_TKS & 0.2015 & 0.2028 \\
%	LM using API (stopped) & \textbf{0.2419} & \textbf{0.2591} \\
%	LM + DRMM & 0.2578 & 0.2620 \\
%	\midrule
%	CC & 0.1816 & 0.1844 \\
%	QE & 0.1645 & 0.1703 \\
%	QLEL & 0.2039 & 0.2002 \\
%	\midrule
%	Features & 0.2600 & 0.2624 \\
%	Features + l & 0.2694 & 0.2692 \\
%	Features + l + l & 0.2867 & 0.2866 \\
%	\midrule
%	LM + cc + DRMM + QE + QLEL  & 0.3417 & 0.3283 \\
%	above + QL & \textbf{0.3518} & \textbf{0.3355} \\
%	above + QL no lm & 0.2895 & 0.2804 \\
%	above + QL + LQ & 0.3476 & 0.3303 \\
%	all mine & 0.2810 & 0.2759 \\
%%	\midrule
%%	Row population & 0.0143 & 0.0599 & 0.0264 \\
%%	Row population (abstract) & 0.0171 & 0.0699 & 0.0277\\
%%	Row population (dbpedia) &&\\
%	\bottomrule	
%	\end{tabular}	
%\label{tbl:er_qs2}
%\end{table}
%
%\begin{table}[t]
%\center
%\caption{Entity retrieval results for query set 2 (ER).}
%	\begin{tabular}{lcc}
%	\toprule
%	\textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
%	\midrule	
%	LM & 0.0708 & 0.0823 \\
%%	CDSSM & & \\
%%	DRMM (5-cross) & 0.0660 & 0.0702 \\
%	DRMM\_TKS & 0.0501 & 0.0540 \\
%	QL & 0.1089 & 0.1083 \\
%	LM + DRMM & 0.0619 & 0.0686 \\
%	LM + drmm + qlel & 0.1417 & 0.1407 \\
%	LM + drmm + QLEL + QL & 0.1426 & 0.1436 \\
%	LQ & 0.1096 & 0.1086 \\
%	LM + drrm + QLEL + QL +LQ & 0.1399 & 0.1426 \\
%	LL & 0.1320 & 0.1318 \\
%	LM + drrm + QLEL + QL +LQ + LL & 0.1403 & 0.1438 \\
%	Above - LQ & 0.1451 & 0.1466 \\
%	Above - LM & 0.1454 & 0.1457 \\
%	ALL DRRM & 0.1182 & 0.1171 \\
%	
%
%%	LM Pair NL query & \textbf{0.0440} & \textbf{0.1403} & \textbf{0.0797} \\
%%	LM Pair Qa query & 0.0259 & 0.0881 & 0.0502 \\
%%	LM Pair Qb query & 0.0240 & 0.0620 & 0.0366 \\
%%	\midrule
%%	Row population (pair) & 0.0101 & 0.0420 & 0.0079 \\
%%	Row population (abstract) &&&\\
%%	Row population (dbpedia)&&&\\
%%	\midrule
%%	LM Triple NL query & 0.0258 & \textbf{0.1192} & 0.0393 \\		
%%	LM Triple Qa query & 0.0096 & 0.0247 & 0.0129 \\	
%%	LM Triple Qb query & 0.0152 & 0.0472 & 0.0237  \\
%%	LM Triple Qc query & 0.0041 & 0.0101 & 0.0038 \\
%%	LM Triple Qab query & \textbf{0.0381} & 0.1028 & \textbf{0.0572} \\
%%	LM Triple Qac query & 0.0180 & 0.0456 & 0.0268 \\
%%	LM Triple Qbc query & 0.0219 & 0.0629 & 0.0314 \\
%%	\midrule
%%	Row population (triple) & 0.0137 & 0.0403 & 0.0116 \\	
%%	Row population (abstract) & 0.0165 & 0.0484 & 0.0154 \\
%%	Row population (dbpedia)&&&\\
%	\bottomrule	
%	\end{tabular}	
%\label{tbl:er_qs1}
%\end{table}
%


\subsection{Schema Determination Evaluation}

\begin{table*}[t]
\center
\caption{Schema determination results for query sets.}
	\begin{tabular}{lccccc}
	\toprule
%	& \multicolumn{5}{c}{\textbf{Query set}} \\
%	 & \multicolumn{2}{c}{\textbf{QS1}} & \multicolumn{2}{c}{\textbf{QS2}} \\
%	 
	 
    	& \multicolumn{2}{c}{\textbf{QS1}} && \multicolumn{2}{c}{\textbf{QS2}} \\
    \cline{2-3} \cline{5-6} 
    \textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} & &
    \textbf{NDCG@5} & \textbf{NDCG@10}  \\
    \midrule

	(1) CP(q) & 0.0561 & 0.0675 && 0.1770 & 0.2092 \\
	(2) TKS\_QS & 0.0380 & 0.0427 && 0.0920 & 0.1415 \\
	(1) + (2) & \textbf{0.0786} & \textbf{0.0878}  && \textbf{0.2310} & \textbf{0.2695} \\
	\midrule
	(3) CP(qE)* & 0.0894 & 0.1073 && 0.1835 & 0.2172 \\
	(4) AR* & 0.0951 & 0.1007 && 0.2419 & 0.2791 \\
	(5) cc* & 0.1470 & 0.2153 && 0.4101 & 0.4739 \\ %DB: cc from only db. ER: cc from tc
	(1) + (2) + (3)* & 0.0996 & 0.1412 && 0.2203 & 0.2562 \\
	(1) + (2) + (4)* & 0.0930 & 0.1021 && 0.2848 & 0.3213 \\
	(1) + (2) + (5)* & 0.1928 & 0.2377 && 0.4169 & 0.4756 \\
	All* & \textbf{0.2002} & \textbf{0.2434} && \textbf{0.4239} & \textbf{0.4825}\\
	\midrule
	round2 top5 & 0.1433 & 0.1804 && 0.3258 & 0.3779 \\
	round2 top10 & 0.1676 & 0.1869 && 0.3342 & 0.3845 \\
	round2 top20 & 0.1580 & 0.1882 && 0.3425 & 0.3929 \\
	\midrule 
	round3 top5 & 0.1648 & 0.1900 && 0.3458 & 0.4034 \\
	round3 top10 & 0.1775 & 0.2046 && 0.3614 & 0.4143 \\
	round3 top20 & 0.1622 & 0.1924 && 0.3697 & 0.4165 \\ % without a
	\bottomrule	
	\end{tabular}	
\label{tbl:sd_qs}
\end{table*}

\begin{table*}[t]
\center
\caption{Schema determination results for query sets.}
	\begin{tabular}{lccccc}
	\toprule
%	& \multicolumn{5}{c}{\textbf{Query set}} \\
%	 & \multicolumn{2}{c}{\textbf{QS1}} & \multicolumn{2}{c}{\textbf{QS2}} \\
%	 
	 
    	& \multicolumn{2}{c}{\textbf{QS1}} && \multicolumn{2}{c}{\textbf{QS2}} \\
    \cline{2-3} \cline{5-6} 
    \textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} & &
    \textbf{NDCG@5} & \textbf{NDCG@10}  \\
    \midrule
	(1) + (2) & 0.0928 & 0.1064  && \textbf{0.2326} & \textbf{0.2710} \\
	\midrule
%	 & & && 0.4672 & 0.5303 \\
%	\midrule
	round2 top5 & 0.1454 & 0.2021 && 0.3720 & 0.4384 \\
	round2 top10 & 0.1663 & 0.2066 && 0.3865 & 0.4638 \\
	round2 top20 & 0.1679 & 0.2112 && 0.3994 & 0.4730 \\
%	\midrule 
%	round3 top5 & 0.1648 & 0.1900 && 0.3716 & 0.4423 \\
%	round3 top10 & 0.1775 & 0.2046 && 0.3889 & 0.4599 \\
%	round3 top20 & 0.1622 & 0.1924 && 0.3987 & 0.4737 \\ % without a
	\bottomrule	
	\end{tabular}	
\label{tbl:sd_qs1}
\end{table*}

%\begin{table}[t]
%\center
%\caption{Schema determination results for DB query set.}
%	\begin{tabular}{lcccc}
%	\toprule
%	\textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
%	\midrule
%	Column population & 0.2315 & 0.2894 \\
%	Column population E & 0.2180 & 0.2759 \\	
%	Attribute retrieval & 0.2246 & 0.2758 \\
%	QL & 0.0962 & 0.1445 \\
%	\bottomrule	
%	\end{tabular}	
%\label{tbl:er_qs1}
%\end{table}
%
%\begin{table}[t]
%\center
%\caption{Schema determination results for ER. (top20)}
%	\begin{tabular}{lcccc}
%	\toprule
%	\textbf{Method} & \textbf{NDCG@5} & \textbf{NDCG@10} \\
%	\midrule
%	Attribut retrieval & 0.2433 & 0.2771 \\
%%	Pair\\
%%	\midrule
%%	Column population q & 0.1002 & 0.2561 & 0.1208 & 0.1512 \\
%%	Column population pc & 0.1463 & 0.3475 & 0.1761 & 0.2102 \\
%%	Attribute retrieval & 0.1793 & 0.4433 & 0.2269 & 0.2552\\
%%	\midrule
%%	Triple\\
%%	\midrule
%%	Column population q & 0.1905 & 0.4423 & 0.2310 & 0.2627  \\
%%	Column population pc & 0.2516 & 0.4896 & 0.2845 & 0.3204  \\	
%%	Attribute retrieval & 0.2210 &  0.4530 & 0.2719 & 0.3151 \\
%	\bottomrule	
%	\end{tabular}	
%\label{tbl:er_qs1}
%\end{table}
